OPD@NL4Opt: An ensemble approach for the NER task of the optimization problem

In this paper, we present an ensemble approach for the NL4Opt competition subtask 1(NER task). For this task, we first fine tune the pretrained language models based on the competition dataset. Then we adopt differential learning rates and adversarial training strategies to enhance the model generalization and robustness. Additionally, we use a model ensemble method for the final prediction, which achieves a micro-averaged F1 score of 93.3% and attains the second prize in the NER task.

==> relate_work.tex <==

\section{Relate Work}
\subsection{Pre-trained language Models}
In recent years, pre-trained language models have achieved remarkable achievement on natural language processing tasks, becoming one of the most effective method for engineers and scholars. Transformers-based Pre-trained language models such as bert\cite{devlin2018bert},  RoBERTa\cite{liu2019roberta}, DEBERTA\citep{he2020deberta},DeBERTaV3\cite{he2021debertav3} is designed to pretrain deep representation from unlabeled text, which  can be fine tuned with just one additional output layer to create state-of-the-art models for a wide range of tasks, such as question answering and language inference, without substantial task specific architecture modifications.


By training language model using Twitter corpora from different time periods, \cite{loureiro2022timelms} showed that language undergoes semantic transformations over time, proving that training a language model with outdated corpora leads to a decline in performance.
\subsection{MOE: Mixture of Experts}
MoE \cite{jiang1999identifiability} is a model architecture for deep learning, which consists of a set of experts, such as neural network models and a trainable gating structure that assign weights to the experts. Given an inputs, the output of MoE is a weighted combination of the experts.Recently,Moe achieves significant improvements on several natural language processing tasks, such as named entity recognition \cite{meng2021gemnet}, recommendation\cite{zhu2020recommendation} and machine translation\citep{shazeer2017outrageously}


